Effects of Non-Vanishing Net Charge in Balance Functions

We investigate the impact of non-vanishing net-charge in collision systems on measurements of balance functions and their integrals. We show that the nominal balance function definition yields integrals that deviate from unity because of the non-vanishing net-charge. However, the integral of unified balance functions is shown to appropriately converge to unity when measured in a sufficiently wide experimental acceptance. We furthermore explore the rate of convergence of unified balance functions integrals and study distortions imparted on the shape of balance functions when measurements are carried out in limited transverse momentum ($p_{\rm T}$) and rapidity ($y$) acceptances, such as those featured by experiments at the Large Hadron Collider or the Relativistic Heavy Ion Collider. We show that the shape and integral of unified balance functions may be strongly biased by reductions in the rapidity and transverse momentum acceptances of existing experiments.

==> Balance Functions_ NetChargeVersion3936-Submission2Archive/defs.tex <==
\newcommand{ \la }{\langle}
\newcommand{ \ra }{\rangle}
\def \mean#1 {{\la #1 \ra}}
\newcommand{ \pp}{pp}
\newcommand{ \pPb}{p -- Pb}
\newcommand{ \PbPb}{Pb -- Pb}
\newcommand{ \AuAu}{Au -- Au}
\newcommand{ \dAu}{d -- Au}
\newcommand{ \ds }{\displaystyle}
\newcommand{\orange}[1]{\textcolor{orange}{#1}}
\newcommand{\blue}[1]{{\color{blue}{#1}}}
\newcommand{\green}[1]{{\color{dgreen}{#1}}}
\newcommand{\red}[1]{{\color{red}{#1}}}
\newcommand{\magenta}[1]{{\color{magenta}{#1}}}


==> defs.tex <==
\newcommand{ \la }{\langle}
\newcommand{ \ra }{\rangle}
\def \mean#1 {{\la #1 \ra}}
\newcommand{ \pp}{pp}
\newcommand{ \pPb}{p -- Pb}
\newcommand{ \PbPb}{Pb -- Pb}
\newcommand{ \AuAu}{Au -- Au}
\newcommand{ \dAu}{d -- Au}
\newcommand{ \ds }{\displaystyle}
\newcommand{\orange}[1]{\textcolor{orange}{#1}}
\newcommand{\blue}[1]{{\color{blue}{#1}}}
\newcommand{\green}[1]{{\color{dgreen}{#1}}}
\newcommand{\red}[1]{{\color{red}{#1}}}
\newcommand{\magenta}[1]{{\color{magenta}{#1}}}

